SDSS-IV MaNGA: Evidence for enriched accretion onto satellite galaxies in dense environments

We investigate the environmental dependence of the local gas-phase metallicity in a sample of star-forming galaxies from the MaNGA survey. Satellite galaxies with stellar masses in the range $9<\log(M_{*}/M_{\odot})<10$ are found to be $\sim 0.05 \, \mathrm{dex}$ higher in metallicity than centrals of similar stellar mass. Within the low-mass satellite population, we find that the interstellar medium (ISM) metallicity depends most strongly on the stellar mass of the galaxy that is central to the halo, though there is no obvious difference in the metallicity gradients. At fixed total stellar mass, the satellites of high mass ($M_{*}>10^{10.5} \, \mathrm{M_{\odot}}$) centrals are $\sim 0.1 \, \mathrm{dex}$ more metal rich than satellites of low-mass ($M_{*} < 10^{10} \, \mathrm{M_{\odot}}$) centrals, controlling for local stellar mass surface density and gas fraction. Fitting a gas-regulator model to the spaxel data, we are able to account for variations in the local gas fraction, stellar mass surface density and local escape velocity-dependent outflows. We find that the best explanation for the metallicity differences is the variation in the average metallicity of accreted gas between different environments that depends on the stellar mass of the dominant galaxies in each halo. This is interpreted as evidence for the exchange of enriched gas between galaxies in dense environments that is predicted by recent simulations.

==> bibliography.tex <==
Automatically generated by Mendeley Desktop 1.19.2
Any changes to this file will be lost if it is regenerated by Mendeley.

BibTeX export options can be customized via Preferences -> BibTeX in Mendeley Desktop

@ARTICLE{Aguado2018,
   author = {{Aguado}, D.~S. and {Ahumada}, R. and {Almeida}, A. and {Anderson}, S.~F. and 
	{Andrews}, B.~H. and {Anguiano}, B. and {Aquino Ortiz}, E. and 
	{Aragon-Salamanca}, A. and {Argudo-Fernandez}, M. and {Aubert}, M. and et al.},
    title = "{The Fifteenth Data Release of the Sloan Digital Sky Surveys: First Release of MaNGA Derived Quantities, Data Visualization Tools and Stellar Library}",
  journal = {arXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1812.02759},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2018,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv181202759A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Alam2015,
   author = {{Alam}, S. and {Albareti}, F.~D. and {Allende Prieto}, C. and 
	{Anders}, F. and {Anderson}, S.~F. and {Anderton}, T. and {Andrews}, B.~H. and 
	{Armengaud}, E. and {Aubourg}, {\'E}. and {Bailey}, S. and et al.},
    title = "{The Eleventh and Twelfth Data Releases of the Sloan Digital Sky Survey: Final Data from SDSS-III}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1501.00963},
 primaryClass = "astro-ph.IM",
 keywords = {atlases, catalogs, surveys},
     year = 2015,
    month = jul,
   volume = 219,
      eid = {12},
    pages = {12},
      doi = {10.1088/0067-0049/219/1/12},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJS..219...12A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AnglesAlcazar2017,
   author = {{Angl{\'e}s-Alc{\'a}zar}, D. and {Faucher-Gigu{\`e}re}, C.-A. and 
	{Kere{\v s}}, D. and {Hopkins}, P.~F. and {Quataert}, E. and 
	{Murray}, N.},
    title = "{The cosmic baryon cycle and galaxy mass assembly in the FIRE simulations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1610.08523},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: star formation, intergalactic medium, cosmology: theory},
     year = 2017,
    month = oct,
   volume = 470,
    pages = {4698-4719},
      doi = {10.1093/mnras/stx1517},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.470.4698A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Astropy2013,
   author = {{Astropy Collaboration} and {Robitaille}, T.~P. and {Tollerud}, E.~J. and 
	{Greenfield}, P. and {Droettboom}, M. and {Bray}, E. and {Aldcroft}, T. and 
	{Davis}, M. and {Ginsburg}, A. and {Price-Whelan}, A.~M. and 
	{Kerzendorf}, W.~E. and {Conley}, A. and {Crighton}, N. and 
	{Barbary}, K. and {Muna}, D. and {Ferguson}, H. and {Grollier}, F. and 
	{Parikh}, M.~M. and {Nair}, P.~H. and {Unther}, H.~M. and {Deil}, C. and 
	{Woillez}, J. and {Conseil}, S. and {Kramer}, R. and {Turner}, J.~E.~H. and 
	{Singer}, L. and {Fox}, R. and {Weaver}, B.~A. and {Zabalza}, V. and 
	{Edwards}, Z.~I. and {Azalee Bostroem}, K. and {Burke}, D.~J. and 
	{Casey}, A.~R. and {Crawford}, S.~M. and {Dencheva}, N. and 
	{Ely}, J. and {Jenness}, T. and {Labrie}, K. and {Lim}, P.~L. and 
	{Pierfederici}, F. and {Pontzen}, A. and {Ptak}, A. and {Refsdal}, B. and 
	{Servillat}, M. and {Streicher}, O.},
    title = "{Astropy: A community Python package for astronomy}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1307.6212},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A33},
    pages = {A33},
      doi = {10.1051/0004-6361/201322068},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2013A%26A...558A..33A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Astropy2018,
   author = {{Astropy Collaboration} and {Price-Whelan}, A.~M. and {Sip{\H o}cz}, B.~M. and 
	{G{\"u}nther}, H.~M. and {Lim}, P.~L. and {Crawford}, S.~M. and 
	{Conseil}, S. and {Shupe}, D.~L. and {Craig}, M.~W. and {Dencheva}, N. and 
	{Ginsburg}, A. and {VanderPlas}, J.~T. and {Bradley}, L.~D. and 
	{P{\'e}rez-Su{\'a}rez}, D. and {de Val-Borro}, M. and {Aldcroft}, T.~L. and 
	{Cruz}, K.~L. and {Robitaille}, T.~P. and {Tollerud}, E.~J. and 
	{Ardelean}, C. and {Babej}, T. and {Bach}, Y.~P. and {Bachetti}, M. and 
	{Bakanov}, A.~V. and {Bamford}, S.~P. and {Barentsen}, G. and 
	{Barmby}, P. and {Baumbach}, A. and {Berry}, K.~L. and {Biscani}, F. and 
	{Boquien}, M. and {Bostroem}, K.~A. and {Bouma}, L.~G. and {Brammer}, G.~B. and 
	{Bray}, E.~M. and {Breytenbach}, H. and {Buddelmeijer}, H. and 
	{Burke}, D.~J. and {Calderone}, G. and {Cano Rodr{\'{\i}}guez}, J.~L. and 
	{Cara}, M. and {Cardoso}, J.~V.~M. and {Cheedella}, S. and {Copin}, Y. and 
	{Corrales}, L. and {Crichton}, D. and {D'Avella}, D. and {Deil}, C. and 
	{Depagne}, {\'E}. and {Dietrich}, J.~P. and {Donath}, A. and 
	{Droettboom}, M. and {Earl}, N. and {Erben}, T. and {Fabbro}, S. and 
	{Ferreira}, L.~A. and {Finethy}, T. and {Fox}, R.~T. and {Garrison}, L.~H. and 
	{Gibbons}, S.~L.~J. and {Goldstein}, D.~A. and {Gommers}, R. and 
	{Greco}, J.~P. and {Greenfield}, P. and {Groener}, A.~M. and 
	{Grollier}, F. and {Hagen}, A. and {Hirst}, P. and {Homeier}, D. and 
	{Horton}, A.~J. and {Hosseinzadeh}, G. and {Hu}, L. and {Hunkeler}, J.~S. and 
	{Ivezi{\'c}}, {\v Z}. and {Jain}, A. and {Jenness}, T. and {Kanarek}, G. and 
	{Kendrew}, S. and {Kern}, N.~S. and {Kerzendorf}, W.~E. and 
	{Khvalko}, A. and {King}, J. and {Kirkby}, D. and {Kulkarni}, A.~M. and 
	{Kumar}, A. and {Lee}, A. and {Lenz}, D. and {Littlefair}, S.~P. and 
	{Ma}, Z. and {Macleod}, D.~M. and {Mastropietro}, M. and {McCully}, C. and 
	{Montagnac}, S. and {Morris}, B.~M. and {Mueller}, M. and {Mumford}, S.~J. and 
	{Muna}, D. and {Murphy}, N.~A. and {Nelson}, S. and {Nguyen}, G.~H. and 
	{Ninan}, J.~P. and {N{\"o}the}, M. and {Ogaz}, S. and {Oh}, S. and 
	{Parejko}, J.~K. and {Parley}, N. and {Pascual}, S. and {Patil}, R. and 
	{Patil}, A.~A. and {Plunkett}, A.~L. and {Prochaska}, J.~X. and 
	{Rastogi}, T. and {Reddy Janga}, V. and {Sabater}, J. and {Sakurikar}, P. and 
	{Seifert}, M. and {Sherbert}, L.~E. and {Sherwood-Taylor}, H. and 
	{Shih}, A.~Y. and {Sick}, J. and {Silbiger}, M.~T. and {Singanamalla}, S. and 
	{Singer}, L.~P. and {Sladen}, P.~H. and {Sooley}, K.~A. and 
	{Sornarajah}, S. and {Streicher}, O. and {Teuben}, P. and {Thomas}, S.~W. and 
	{Tremblay}, G.~R. and {Turner}, J.~E.~H. and {Terr{\'o}n}, V. and 
	{van Kerkwijk}, M.~H. and {de la Vega}, A. and {Watkins}, L.~L. and 
	{Weaver}, B.~A. and {Whitmore}, J.~B. and {Woillez}, J. and 
	{Zabalza}, V. and {Astropy Contributors}},
    title = "{The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1801.02634},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, methods: statistical, reference systems},
     year = 2018,
    month = sep,
   volume = 156,
      eid = {123},
    pages = {123},
      doi = {10.3847/1538-3881/aabc4f},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..123A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Baldwin1981,
   author = {{Baldwin}, J.~A. and {Phillips}, M.~M. and {Terlevich}, R.},
    title = "{Classification parameters for the emission-line spectra of extragalactic objects}",
  journal = {\pasp},
 keywords = {Astronomical Spectroscopy, Emission Spectra, Line Spectra, Quasars, Seyfert Galaxies, Classifications, H Ii Regions, Photoionization, Planetary Nebulae, Shock Heating},
     year = 1981,
    month = feb,
   volume = 93,
    pages = {5-19},
      doi = {10.1086/130766},
   adsurl = {http://adsabs.harvard.edu/abs/1981PASP...93....5B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BarreraBallesteros2014,
   author = {{Barrera-Ballesteros}, J.~K. and {Falc{\'o}n-Barroso}, J. and 
	{Garc{\'{\i}}a-Lorenzo}, B. and {van de Ven}, G. and {Aguerri}, J.~A.~L. and 
	{Mendez-Abreu}, J. and {Spekkens}, K. and {Lyubenova}, M. and 
	{S{\'a}nchez}, S.~F. and {Husemann}, B. and {Mast}, D. and {Garc{\'{\i}}a-Benito}, R. and 
	{Iglesias-Paramo}, J. and {Del Olmo}, A. and {M{\'a}rquez}, I. and 
	{Masegosa}, J. and {Kehrig}, C. and {Marino}, R.~A. and {Verdes-Montenegro}, L. and 
	{Ziegler}, B. and {McIntosh}, D.~H. and {Bland-Hawthorn}, J. and 
	{Walcher}, C.~J. and {Califa Collaboration}},
    title = "{Kinematic alignment of non-interacting CALIFA galaxies. Quantifying the impact of bars on stellar and ionised gas velocity field orientations}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1405.5222},
 keywords = {galaxies: kinematics and dynamics, galaxies: photometry, galaxies: structure, galaxies: evolution},
     year = 2014,
    month = aug,
   volume = 568,
      eid = {A70},
    pages = {A70},
      doi = {10.1051/0004-6361/201423488},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...568A..70B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BarreraBallesteros2016,
       author = {{Barrera-Ballesteros}, Jorge K. and {Heckman}, Timothy M. and
         {Zhu}, Guangtun B. and {Zakamska}, Nadia L. and
         {S{\'a}nchez}, Sebastian F. and {Law}, David and {Wake}, David and
         {Green}, Jenny E. and {Bizyaev}, Dmitry and {Oravetz}, Daniel and
         {Simmons}, Audrey and {Malanushenko}, Elena and {Pan}, Kaike and
         {Roman Lopes}, Alexandre and {Lane}, Richard R.},
        title = "{Do galaxy global relationships emerge from local ones? The SDSS IV MaNGA surface mass density-metallicity relation}",
      journal = {\mnras},
     keywords = {techniques: imaging spectroscopy, galaxies: abundances, galaxies: fundamental parameters, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Dec",
       volume = {463},
       number = {3},
        pages = {2513-2522},
          doi = {10.1093/mnras/stw1984},
archivePrefix = {arXiv},
       eprint = {1609.01740},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.463.2513B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BarreraBallesteros2018,
   author = {{Barrera-Ballesteros}, J.~K. and {Heckman}, T. and {S{\'a}nchez}, S.~F. and 
	{Zakamska}, N.~L. and {Cleary}, J. and {Zhu}, G. and {Brinkmann}, J. and 
	{Drory}, N. and {THE MaNGA TEAM}},
    title = "{SDSS-IV MaNGA: What Shapes the Distribution of Metals in Galaxies? Exploring the Roles of the Local Gas Fraction and Escape Velocity}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1711.10492},
 keywords = {galaxies: abundances, galaxies: evolution, galaxies: kinematics and dynamics, galaxies: statistics, surveys, techniques: imaging spectroscopy},
     year = 2018,
    month = jan,
   volume = 852,
      eid = {74},
    pages = {74},
      doi = {10.3847/1538-4357/aa9b31},
   adsurl = {http://adsabs.harvard.edu/abs/2018ApJ...852...74B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Behroozi2010,
   author = {{Behroozi}, P.~S. and {Conroy}, C. and {Wechsler}, R.~H.},
    title = "{A Comprehensive Analysis of Uncertainties Affecting the Stellar Mass-Halo Mass Relation for 0 $\lt$ z $\lt$ 4}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1001.0015},
 primaryClass = "astro-ph.CO",
 keywords = {dark matter, galaxies: abundances, galaxies: evolution, galaxies: stellar content},
     year = 2010,
    month = jul,
   volume = 717,
    pages = {379-403},
      doi = {10.1088/0004-637X/717/1/379},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...717..379B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Belfiore2017,
   author = {{Belfiore}, F. and {Maiolino}, R. and {Tremonti}, C. and {S{\'a}nchez}, S.~F. and 
	{Bundy}, K. and {Bershady}, M. and {Westfall}, K. and {Lin}, L. and 
	{Drory}, N. and {Boquien}, M. and {Thomas}, D. and {Brinkmann}, J.
	},
    title = "{SDSS IV MaNGA - metallicity and nitrogen abundance gradients in local galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1703.03813},
 keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: ISM},
     year = 2017,
    month = jul,
   volume = 469,
    pages = {151-170},
      doi = {10.1093/mnras/stx789},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.469..151B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Belfiore2019,
   author = {{Belfiore}, F. and {Westfall}, K.~B. and {Schaefer}, A. and 
	{Cappellari}, M. and {Ji}, X. and {Bershady}, M.~A. and {Tremonti}, C. and 
	{Law}, D.~R. and {Yan}, R. and {Bundy}, K. and {Shetty}, S. and 
	{Drory}, N. and {Thomas}, D. and {Emsellem}, E. and {S{\'a}nchez}, S.~F.
	},
    title = "{The Data Analysis Pipeline for the SDSS-IV MaNGA IFU Galaxy Survey: Emission-Line Modeling}",
  journal = {arXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1901.00866},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2019,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2019arXiv190100866B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bigiel2008,
   author = {{Bigiel}, F. and {Leroy}, A. and {Walter}, F. and {Brinks}, E. and 
	{de Blok}, W.~J.~G. and {Madore}, B. and {Thornley}, M.~D.},
    title = "{The Star Formation Law in Nearby Galaxies on Sub-Kpc Scales}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0810.2541},
 keywords = {galaxies: evolution, galaxies: ISM, radio lines: galaxies, radio lines: ISM},
     year = 2008,
    month = dec,
   volume = 136,
    pages = {2846-2871},
      doi = {10.1088/0004-6256/136/6/2846},
   adsurl = {http://adsabs.harvard.edu/abs/2008AJ....136.2846B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Birnboim2003,
       author = {{Birnboim}, Yuval and {Dekel}, Avishai},
        title = "{Virial shocks in galactic haloes?}",
      journal = {\mnras},
     keywords = {hydrodynamics, shock waves, cooling flows, galaxies: formation, galaxies: ISM, dark matter, Astrophysics},
         year = "2003",
        month = "Oct",
       volume = {345},
       number = {1},
        pages = {349-364},
          doi = {10.1046/j.1365-8711.2003.06955.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0302161},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003MNRAS.345..349B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Blanc2015,
   author = {{Blanc}, G.~A. and {Kewley}, L. and {Vogt}, F.~P.~A. and {Dopita}, M.~A.
	},
    title = "{IZI: Inferring the Gas Phase Metallicity (Z) and Ionization Parameter (q) of Ionized Nebulae Using Bayesian Statistics}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1410.8146},
 keywords = {astrochemistry, galaxies: abundances, galaxies: ISM, H II regions, ISM: abundances},
     year = 2015,
    month = jan,
   volume = 798,
      eid = {99},
    pages = {99},
      doi = {10.1088/0004-637X/798/2/99},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798...99B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Blanton2011,
       author = {{Blanton}, Michael R. and {Kazin}, Eyal and {Muna}, Demitri and
         {Weaver}, Benjamin A. and {Price-Whelan}, Adrian},
        title = "{Improved Background Subtraction for the Sloan Digital Sky Survey Images}",
      journal = {\aj},
     keywords = {atmospheric effects, galaxies: photometry, methods: data analysis, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2011",
        month = "Jul",
       volume = {142},
       number = {1},
          eid = {31},
        pages = {31},
          doi = {10.1088/0004-6256/142/1/31},
archivePrefix = {arXiv},
       eprint = {1105.1960},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AJ....142...31B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bohm2004,
   author = {{B{\"o}hm}, A. and {Ziegler}, B.~L. and {Saglia}, R.~P. and 
	{Bender}, R. and {Fricke}, K.~J. and {Gabasch}, A. and {Heidt}, J. and 
	{Mehlert}, D. and {Noll}, S. and {Seitz}, S.},
    title = "{The Tully-Fisher relation at intermediate redshift}",
  journal = {\aap},
   eprint = {astro-ph/0309263},
 keywords = {galaxies: spiral, galaxies: evolution, galaxies: kinematics and dynamics},
     year = 2004,
    month = jun,
   volume = 420,
    pages = {97-114},
      doi = {10.1051/0004-6361:20034256},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...420...97B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bothwell2013,
   author = {{Bothwell}, M.~S. and {Maiolino}, R. and {Kennicutt}, R. and 
	{Cresci}, G. and {Mannucci}, F. and {Marconi}, A. and {Cicone}, C.
	},
    title = "{A fundamental relation between the metallicity, gas content and stellar mass of local galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1304.4940},
 keywords = {galaxies: abundances, galaxies: evolution, galaxies: formation, galaxies: statistics},
     year = 2013,
    month = aug,
   volume = 433,
    pages = {1425-1435},
      doi = {10.1093/mnras/stt817},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433.1425B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brook2014,
       author = {{Brook}, C.~B. and {Stinson}, G. and {Gibson}, B.~K. and {Shen}, S. and
         {Macci{\`o}}, A.~V. and {Obreja}, A. and {Wadsley}, J. and {Quinn}, T.},
        title = "{MaGICC baryon cycle: the enrichment history of simulated disc galaxies}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: spiral, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2014",
        month = "Oct",
       volume = {443},
       number = {4},
        pages = {3809-3818},
          doi = {10.1093/mnras/stu1406},
archivePrefix = {arXiv},
       eprint = {1306.5766},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.443.3809B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bruzual2003,
   author = {{Bruzual}, G. and {Charlot}, S.},
    title = "{Stellar population synthesis at the resolution of 2003}",
  journal = {\mnras},
   eprint = {astro-ph/0309134},
 keywords = {stars: evolution, galaxies: evolution, galaxies: formation, galaxies: stellar content},
     year = 2003,
    month = oct,
   volume = 344,
    pages = {1000-1028},
      doi = {10.1046/j.1365-8711.2003.06897.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.344.1000B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bryant2015,
   author = {{Bryant}, J.~J. and {Owers}, M.~S. and {Robotham}, A.~S.~G. and 
	{Croom}, S.~M. and {Driver}, S.~P. and {Drinkwater}, M.~J. and 
	{Lorente}, N.~P.~F. and {Cortese}, L. and {Scott}, N. and {Colless}, M. and 
	{Schaefer}, A. and {Taylor}, E.~N. and {Konstantopoulos}, I.~S. and 
	{Allen}, J.~T. and {Baldry}, I. and {Barnes}, L. and {Bauer}, A.~E. and 
	{Bland-Hawthorn}, J. and {Bloom}, J.~V. and {Brooks}, A.~M. and 
	{Brough}, S. and {Cecil}, G. and {Couch}, W. and {Croton}, D. and 
	{Davies}, R. and {Ellis}, S. and {Fogarty}, L.~M.~R. and {Foster}, C. and 
	{Glazebrook}, K. and {Goodwin}, M. and {Green}, A. and {Gunawardhana}, M.~L. and 
	{Hampton}, E. and {Ho}, I.-T. and {Hopkins}, A.~M. and {Kewley}, L. and 
	{Lawrence}, J.~S. and {Leon-Saval}, S.~G. and {Leslie}, S. and 
	{McElroy}, R. and {Lewis}, G. and {Liske}, J. and {L{\'o}pez-S{\'a}nchez}, {\'A}.~R. and 
	{Mahajan}, S. and {Medling}, A.~M. and {Metcalfe}, N. and {Meyer}, M. and 
	{Mould}, J. and {Obreschkow}, D. and {O'Toole}, S. and {Pracy}, M. and 
	{Richards}, S.~N. and {Shanks}, T. and {Sharp}, R. and {Sweet}, S.~M. and 
	{Thomas}, A.~D. and {Tonini}, C. and {Walcher}, C.~J.},
    title = "{The SAMI Galaxy Survey: instrument specification and target selection}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1407.7335},
 keywords = {instrumentation: miscellaneous, instrumentation: spectrographs, techniques: imaging spectroscopy, surveys, galaxies: evolution, galaxies: kinematics and dynamics},
     year = 2015,
    month = mar,
   volume = 447,
    pages = {2857-2879},
      doi = {10.1093/mnras/stu2635},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.447.2857B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Bryant2016,
       author = {{Bryant}, Julia J. and {Bland-Hawthorn}, Joss and {Lawrence}, Jon and
         {Croom}, Scott and {Brown}, David and {Venkatesan}, Sudharshan and
         {Gillingham}, Peter R. and {Zhelem}, Ross and {Content}, Robert and
         {Saunders}, Will and {Staszak}, Nicholas F. and {van de Sande}, Jesse and
         {Couch}, Warrick and {Leon-Saval}, Sergio and {Tims}, Julia and
         {McDermid}, Richard and {Schaefer}, Adam},
        title = "{Hector: a new massively multiplexed IFU instrument for the Anglo-Australian Telescope}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy VI},
         year = "2016",
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9908},
        month = "Aug",
          eid = {99081F},
        pages = {99081F},
          doi = {10.1117/12.2230740},
archivePrefix = {arXiv},
       eprint = {1608.03921},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016SPIE.9908E..1FB},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bundy2015,
   author = {{Bundy}, K. and {Bershady}, M.~A. and {Law}, D.~R. and {Yan}, R. and 
	{Drory}, N. and {MacDonald}, N. and {Wake}, D.~A. and {Cherinka}, B. and 
	{S{\'a}nchez-Gallego}, J.~R. and {Weijmans}, A.-M. and {Thomas}, D. and 
	{Tremonti}, C. and {Masters}, K. and {Coccato}, L. and {Diamond-Stanic}, A.~M. and 
	{Arag{\'o}n-Salamanca}, A. and {Avila-Reese}, V. and {Badenes}, C. and 
	{Falc{\'o}n-Barroso}, J. and {Belfiore}, F. and {Bizyaev}, D. and 
	{Blanc}, G.~A. and {Bland-Hawthorn}, J. and {Blanton}, M.~R. and 
	{Brownstein}, J.~R. and {Byler}, N. and {Cappellari}, M. and 
	{Conroy}, C. and {Dutton}, A.~A. and {Emsellem}, E. and {Etherington}, J. and 
	{Frinchaboy}, P.~M. and {Fu}, H. and {Gunn}, J.~E. and {Harding}, P. and 
	{Johnston}, E.~J. and {Kauffmann}, G. and {Kinemuchi}, K. and 
	{Klaene}, M.~A. and {Knapen}, J.~H. and {Leauthaud}, A. and 
	{Li}, C. and {Lin}, L. and {Maiolino}, R. and {Malanushenko}, V. and 
	{Malanushenko}, E. and {Mao}, S. and {Maraston}, C. and {McDermid}, R.~M. and 
	{Merrifield}, M.~R. and {Nichol}, R.~C. and {Oravetz}, D. and 
	{Pan}, K. and {Parejko}, J.~K. and {Sanchez}, S.~F. and {Schlegel}, D. and 
	{Simmons}, A. and {Steele}, O. and {Steinmetz}, M. and {Thanjavur}, K. and 
	{Thompson}, B.~A. and {Tinker}, J.~L. and {van den Bosch}, R.~C.~E. and 
	{Westfall}, K.~B. and {Wilkinson}, D. and {Wright}, S. and {Xiao}, T. and 
	{Zhang}, K.},
    title = "{Overview of the SDSS-IV MaNGA Survey: Mapping nearby Galaxies at Apache Point Observatory}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1412.1482},
 keywords = {galaxies: evolution, galaxies: general, surveys, techniques: imaging spectroscopy},
     year = 2015,
    month = jan,
   volume = 798,
      eid = {7},
    pages = {7},
      doi = {10.1088/0004-637X/798/1/7},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798....7B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CanoDiaz2016,
   author = {{Cano-D{\'{\i}}az}, M. and {S{\'a}nchez}, S.~F. and {Zibetti}, S. and 
	{Ascasibar}, Y. and {Bland-Hawthorn}, J. and {Ziegler}, B. and 
	{Gonz{\'a}lez Delgado}, R.~M. and {Walcher}, C.~J. and {Garc{\'{\i}}a-Benito}, R. and 
	{Mast}, D. and {Mendoza-P{\'e}rez}, M.~A. and {Falc{\'o}n-Barroso}, J. and 
	{Galbany}, L. and {Husemann}, B. and {Kehrig}, C. and {Marino}, R.~A. and 
	{S{\'a}nchez-Bl{\'a}zquez}, P. and {L{\'o}pez-Cob{\'a}}, C. and 
	{L{\'o}pez-S{\'a}nchez}, {\'A}.~R. and {Vilchez}, J.~M.},
    title = "{Spatially Resolved Star Formation Main Sequence of Galaxies in the CALIFA Survey}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1602.02770},
 keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: star formation},
     year = 2016,
    month = apr,
   volume = 821,
      eid = {L26},
    pages = {L26},
      doi = {10.3847/2041-8205/821/2/L26},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...821L..26C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari2003,
   author = {{Cappellari}, M. and {Copin}, Y.},
    title = "{Adaptive spatial binning of integral-field spectroscopic data using Voronoi tessellations}",
  journal = {\mnras},
   eprint = {astro-ph/0302262},
 keywords = {methods: data analysis, techniques: photometric, techniques: spectroscopic},
     year = 2003,
    month = jun,
   volume = 342,
    pages = {345-354},
      doi = {10.1046/j.1365-8711.2003.06541.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.342..345C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari2004,
   author = {{Cappellari}, M. and {Emsellem}, E.},
    title = "{Parametric Recovery of Line-of-Sight Velocity Distributions from Absorption-Line Spectra of Galaxies via Penalized Likelihood}",
  journal = {\pasp},
   eprint = {astro-ph/0312201},
 keywords = {Galaxies: Individual: NGC Number: NGC 3384, Galaxies: Kinematics and Dynamics, line: profiles, Methods: Numerical},
     year = 2004,
    month = feb,
   volume = 116,
    pages = {138-147},
      doi = {10.1086/381875},
   adsurl = {http://adsabs.harvard.edu/abs/2004PASP..116..138C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cardelli1989,
   author = {{Cardelli}, J.~A. and {Clayton}, G.~C. and {Mathis}, J.~S.},
    title = "{The relationship between infrared, optical, and ultraviolet extinction}",
  journal = {\apj},
 keywords = {Infrared Spectra, Interstellar Extinction, Ultraviolet Spectra, Visible Spectrum, Computational Astrophysics, Interstellar Matter, Iue},
     year = 1989,
    month = oct,
   volume = 345,
    pages = {245-256},
      doi = {10.1086/167900},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...345..245C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Carton2015,
   author = {{Carton}, D. and {Brinchmann}, J. and {Wang}, J. and {Bigiel}, F. and 
	{Cormier}, D. and {van der Hulst}, T. and {J{\'o}zsa}, G.~I.~G. and 
	{Serra}, P. and {Verheijen}, M.~A.~W.},
    title = "{Gas-phase metallicity profiles of the Bluedisk galaxies: Is metallicity in a local star formation regulated equilibrium?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1505.02797},
 keywords = {galaxies: abundances, galaxies: evolution, galaxies: ISM},
     year = 2015,
    month = jul,
   volume = 451,
    pages = {210-235},
      doi = {10.1093/mnras/stv967},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.451..210C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Carton2017,
       author = {{Carton}, David and {Brinchmann}, Jarle and {Shirazi}, Maryam and
         {Contini}, Thierry and {Epinat}, Beno{\^\i}t and
         {Erroz-Ferrer}, Santiago and {Marino}, Raffaella A. and
         {Martinsson}, Thomas P.~K. and {Richard}, Johan and
         {Patr{\'\i}cio}, Vera},
        title = "{Inferring gas-phase metallicity gradients of galaxies at the seeing limit: a forward modelling approach}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: evolution, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Jun",
       volume = {468},
       number = {2},
        pages = {2140-2163},
          doi = {10.1093/mnras/stx545},
archivePrefix = {arXiv},
       eprint = {1703.01090},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.468.2140C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chabrier2003,
   author = {{Chabrier}, G.},
    title = "{Galactic Stellar and Substellar Initial Mass Function}",
  journal = {\pasp},
   eprint = {astro-ph/0304382},
 keywords = {Galaxies: Luminosity Function, Mass Function, Invited Reviews},
     year = 2003,
    month = jul,
   volume = 115,
    pages = {763-795},
      doi = {10.1086/376392},
   adsurl = {http://adsabs.harvard.edu/abs/2003PASP..115..763C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Charlot2000,
       author = {{Charlot}, St{\'e}phane and {Fall}, S. Michael},
        title = "{A Simple Model for the Absorption of Starlight by Dust in Galaxies}",
      journal = {\apj},
     keywords = {ISM: Dust, Extinction, Galaxies: ISM, Galaxies: Starburst, Infrared: Galaxies, Ultraviolet: Galaxies, Astrophysics},
         year = "2000",
        month = "Aug",
       volume = {539},
       number = {2},
        pages = {718-731},
          doi = {10.1086/309250},
archivePrefix = {arXiv},
       eprint = {astro-ph/0003128},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...539..718C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chisholm2018,
   author = {{Chisholm}, J. and {Tremonti}, C. and {Leitherer}, C.},
    title = "{Metal-enriched galactic outflows shape the mass-metallicity relationship}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1808.10453},
 keywords = {ISM: jets and outflows, galaxies: evolution, galaxies: formation, ultraviolet: ISM},
     year = 2018,
    month = dec,
   volume = 481,
    pages = {1690-1706},
      doi = {10.1093/mnras/sty2380},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.481.1690C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CidFernandes2013,
       author = {{Cid Fernandes}, R. and {P{\'e}rez}, E. and {Garc{\'\i}a Benito}, R. and
         {Gonz{\'a}lez Delgado}, R.~M. and {de Amorim}, A.~L. and
         {S{\'a}nchez}, S.~F. and {Husemann}, B. and {Falc{\'o}n Barroso}, J. and
         {S{\'a}nchez-Bl{\'a}zquez}, P. and {Walcher}, C.~J. and {Mast}, D.},
        title = "{Resolving galaxies in time and space. I. Applying STARLIGHT to CALIFA datacubes}",
      journal = {\aap},
     keywords = {galaxies: general, galaxies: stellar content, galaxies: fundamental parameters, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2013",
        month = "Sep",
       volume = {557},
          eid = {A86},
        pages = {A86},
          doi = {10.1051/0004-6361/201220616},
archivePrefix = {arXiv},
       eprint = {1304.5788},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...557A..86C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Cooper2008,
   author = {{Cooper}, M.~C. and {Tremonti}, C.~A. and {Newman}, J.~A. and 
	{Zabludoff}, A.~I.},
    title = "{The role of environment in the mass-metallicity relation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0805.0308},
 keywords = {galaxies: abundances , galaxies: evolution , galaxies: fundamental parameters , galaxies: statistics , large-scale structure of Universe},
     year = 2008,
    month = oct,
   volume = 390,
    pages = {245-256},
      doi = {10.1111/j.1365-2966.2008.13714.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390..245C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Courteau1997,
   author = {{Courteau}, S.},
    title = "{Optical Rotation Curves and Linewidths for Tully-Fisher Applications}",
  journal = {\aj},
   eprint = {astro-ph/9709201},
 keywords = {GALAXIES: SPIRAL, GALAXIES: KINEMATICS AND DYNAMICS, LOCAL GROUP, GALAXIES: FUNDAMENTAL PARAMETERS},
     year = 1997,
    month = dec,
   volume = 114,
    pages = {2402},
      doi = {10.1086/118656},
   adsurl = {http://adsabs.harvard.edu/abs/1997AJ....114.2402C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Croom2012,
   author = {{Croom}, S.~M. and {Lawrence}, J.~S. and {Bland-Hawthorn}, J. and 
	{Bryant}, J.~J. and {Fogarty}, L. and {Richards}, S. and {Goodwin}, M. and 
	{Farrell}, T. and {Miziarski}, S. and {Heald}, R. and {Jones}, D.~H. and 
	{Lee}, S. and {Colless}, M. and {Brough}, S. and {Hopkins}, A.~M. and 
	{Bauer}, A.~E. and {Birchall}, M.~N. and {Ellis}, S. and {Horton}, A. and 
	{Leon-Saval}, S. and {Lewis}, G. and {L{\'o}pez-S{\'a}nchez}, {\'A}.~R. and 
	{Min}, S.-S. and {Trinh}, C. and {Trowland}, H.},
    title = "{The Sydney-AAO Multi-object Integral field spectrograph}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1112.3367},
 keywords = {instrumentation: spectrographs, techniques: imaging spectroscopy, surveys, galaxies: general, galaxies: kinematics and dynamics},
     year = 2012,
    month = mar,
   volume = 421,
    pages = {872-893},
      doi = {10.1111/j.1365-2966.2011.20365.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421..872C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Davies2016,
   author = {{Davies}, L.~J.~M. and {Robotham}, A.~S.~G. and {Driver}, S.~P. and 
	{Alpaslan}, M. and {Baldry}, I.~K. and {Bland-Hawthorn}, J. and 
	{Brough}, S. and {Brown}, M.~J.~I. and {Cluver}, M.~E. and {Holwerda}, B.~W. and 
	{Hopkins}, A.~M. and {Lara-L{\'o}pez}, M.~A. and {Mahajan}, S. and 
	{Moffett}, A.~J. and {Owers}, M.~S. and {Phillipps}, S.},
    title = "{Galaxy And Mass Assembly (GAMA): growing up in a bad neighbourhood - how do low-mass galaxies become passive?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1511.02245},
 keywords = {galaxies: evolution, galaxies: interactions},
     year = 2016,
    month = feb,
   volume = 455,
    pages = {4013-4029},
      doi = {10.1093/mnras/stv2573},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.455.4013D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{D'Eugenio2018,
   author = {{D'Eugenio}, F. and {Colless}, M. and {Groves}, B. and {Bian}, F. and 
	{Barone}, T.~M.},
    title = "{The gas-phase metallicities of star-forming galaxies in aperture-matched SDSS samples follow potential rather than mass or average surface density}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1805.12131},
 keywords = {galaxies: abundances, galaxies: evolution, galaxies: fundamental parameters},
     year = 2018,
    month = sep,
   volume = 479,
    pages = {1807-1821},
      doi = {10.1093/mnras/sty1424},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.479.1807D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dopita2016,
   author = {{Dopita}, M.~A. and {Kewley}, L.~J. and {Sutherland}, R.~S. and 
	{Nicholls}, D.~C.},
    title = "{Chemical abundances in high-redshift galaxies: a powerful new emission line diagnostic}",
  journal = {\apss},
archivePrefix = "arXiv",
   eprint = {1601.01337},
 keywords = {Galaxies: high redshift, Galaxies: chemical abundances, HII regions, Emission lines},
     year = 2016,
    month = feb,
   volume = 361,
      eid = {61},
    pages = {61},
      doi = {10.1007/s10509-016-2657-8},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016Ap%26SS.361...61D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eisenstein2011,
   author = {{Eisenstein}, D.~J. and {Weinberg}, D.~H. and {Agol}, E. and 
	{Aihara}, H. and {Allende Prieto}, C. and {Anderson}, S.~F. and 
	{Arns}, J.~A. and {Aubourg}, {\'E}. and {Bailey}, S. and {Balbinot}, E. and et al.},
    title = "{SDSS-III: Massive Spectroscopic Surveys of the Distant Universe, the Milky Way, and Extra-Solar Planetary Systems}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1101.1529},
 primaryClass = "astro-ph.IM",
 keywords = {cosmology: observations, Galaxy: evolution, planets and satellites: detection, surveys},
     year = 2011,
    month = sep,
   volume = 142,
      eid = {72},
    pages = {72},
      doi = {10.1088/0004-6256/142/3/72},
   adsurl = {http://adsabs.harvard.edu/abs/2011AJ....142...72E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Erb2008,
   author = {{Erb}, D.~K.},
    title = "{A Model for Star Formation, Gas Flows, and Chemical Evolution in Galaxies at High Redshifts}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0710.4146},
 keywords = {galaxies: abundances, galaxies: evolution, galaxies: high-redshift},
     year = 2008,
    month = feb,
   volume = 674,
    pages = {151-156},
      doi = {10.1086/524727},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...674..151E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{FalconBarroso2011,
   author = {{Falc{\'o}n-Barroso}, J. and {S{\'a}nchez-Bl{\'a}zquez}, P. and 
	{Vazdekis}, A. and {Ricciardelli}, E. and {Cardiel}, N. and 
	{Cenarro}, A.~J. and {Gorgas}, J. and {Peletier}, R.~F.},
    title = "{An updated MILES stellar library and stellar population models}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1107.2303},
 keywords = {catalogs, methods: data analysis, techniques: spectroscopic, stars: kinematics and dynamics, galaxies: kinematics and dynamics},
     year = 2011,
    month = aug,
   volume = 532,
      eid = {A95},
    pages = {A95},
      doi = {10.1051/0004-6361/201116842},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...532A..95F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fielding2017,
       author = {{Fielding}, Drummond and {Quataert}, Eliot and {McCourt}, Michael and
         {Thompson}, Todd A.},
        title = "{The impact of star formation feedback on the circumgalactic medium}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: haloes, intergalactic medium, quasars: absorption lines, cosmology: theory, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2017",
        month = "Apr",
       volume = {466},
       number = {4},
        pages = {3810-3826},
          doi = {10.1093/mnras/stw3326},
archivePrefix = {arXiv},
       eprint = {1606.06734},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.466.3810F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Finlator2008,
   author = {{Finlator}, K. and {Dav{\'e}}, R.},
    title = "{The origin of the galaxy mass-metallicity relation and implications for galactic outflows}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0704.3100},
 keywords = {galaxies: abundances , galaxies: evolution , cosmology: theory},
     year = 2008,
    month = apr,
   volume = 385,
    pages = {2181-2204},
      doi = {10.1111/j.1365-2966.2008.12991.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385.2181F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Finlator2017,
       author = {{Finlator}, Kristian},
        title = "{Gas Accretion and Galactic Chemical Evolution: Theory and Observations}",
     keywords = {Physics, Astrophysics - Astrophysics of Galaxies},
    booktitle = {Gas Accretion onto Galaxies},
         year = "2017",
       editor = {{Fox}, Andrew and {Dav{\'e}}, Romeel},
       series = {Astrophysics and Space Science Library},
       volume = {430},
        month = "Jan",
        pages = {221},
          doi = {10.1007/978-3-319-52512-9_10},
archivePrefix = {arXiv},
       eprint = {1612.00802},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ASSL..430..221F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gunawardhana2011,
   author = {{Gunawardhana}, M.~L.~P. and {Hopkins}, A.~M. and {Sharp}, R.~G. and 
	{Brough}, S. and {Taylor}, E. and {Bland-Hawthorn}, J. and {Maraston}, C. and 
	{Tuffs}, R.~J. and {Popescu}, C.~C. and {Wijesinghe}, D. and 
	{Jones}, D.~H. and {Croom}, S. and {Sadler}, E. and {Wilkins}, S. and 
	{Driver}, S.~P. and {Liske}, J. and {Norberg}, P. and {Baldry}, I.~K. and 
	{Bamford}, S.~P. and {Loveday}, J. and {Peacock}, J.~A. and 
	{Robotham}, A.~S.~G. and {Zucker}, D.~B. and {Parker}, Q.~A. and 
	{Conselice}, C.~J. and {Cameron}, E. and {Frenk}, C.~S. and 
	{Hill}, D.~T. and {Kelvin}, L.~S. and {Kuijken}, K. and {Madore}, B.~F. and 
	{Nichol}, B. and {Parkinson}, H.~R. and {Pimbblet}, K.~A. and 
	{Prescott}, M. and {Sutherland}, W.~J. and {Thomas}, D. and 
	{van Kampen}, E.},
    title = "{Galaxy and Mass Assembly (GAMA): the star formation rate dependence of the stellar initial mass function}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1104.2379},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: star formation, galaxies: stellar content},
     year = 2011,
    month = aug,
   volume = 415,
    pages = {1647-1662},
      doi = {10.1111/j.1365-2966.2011.18800.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.415.1647G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gunn1972,
   author = {{Gunn}, J.~E. and {Gott}, III, J.~R.},
    title = "{On the Infall of Matter Into Clusters of Galaxies and Some Effects on Their Evolution}",
  journal = {\apj},
     year = 1972,
    month = aug,
   volume = 176,
    pages = {1},
      doi = {10.1086/151605},
   adsurl = {http://adsabs.harvard.edu/abs/1972ApJ...176....1G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gunn2006,
   author = {{Gunn}, J.~E. and {Siegmund}, W.~A. and {Mannery}, E.~J. and 
	{Owen}, R.~E. and {Hull}, C.~L. and {Leger}, R.~F. and {Carey}, L.~N. and 
	{Knapp}, G.~R. and {York}, D.~G. and {Boroski}, W.~N. and {Kent}, S.~M. and 
	{Lupton}, R.~H. and {Rockosi}, C.~M. and {Evans}, M.~L. and 
	{Waddell}, P. and {Anderson}, J.~E. and {Annis}, J. and {Barentine}, J.~C. and 
	{Bartoszek}, L.~M. and {Bastian}, S. and {Bracker}, S.~B. and 
	{Brewington}, H.~J. and {Briegel}, C.~I. and {Brinkmann}, J. and 
	{Brown}, Y.~J. and {Carr}, M.~A. and {Czarapata}, P.~C. and 
	{Drennan}, C.~C. and {Dombeck}, T. and {Federwitz}, G.~R. and 
	{Gillespie}, B.~A. and {Gonzales}, C. and {Hansen}, S.~U. and 
	{Harvanek}, M. and {Hayes}, J. and {Jordan}, W. and {Kinney}, E. and 
	{Klaene}, M. and {Kleinman}, S.~J. and {Kron}, R.~G. and {Kresinski}, J. and 
	{Lee}, G. and {Limmongkol}, S. and {Lindenmeyer}, C.~W. and 
	{Long}, D.~C. and {Loomis}, C.~L. and {McGehee}, P.~M. and {Mantsch}, P.~M. and 
	{Neilsen}, Jr., E.~H. and {Neswold}, R.~M. and {Newman}, P.~R. and 
	{Nitta}, A. and {Peoples}, Jr., J. and {Pier}, J.~R. and {Prieto}, P.~S. and 
	{Prosapio}, A. and {Rivetta}, C. and {Schneider}, D.~P. and 
	{Snedden}, S. and {Wang}, S.-i.},
    title = "{The 2.5 m Telescope of the Sloan Digital Sky Survey}",
  journal = {\aj},
   eprint = {astro-ph/0602326},
 keywords = {Surveys, Telescopes},
     year = 2006,
    month = apr,
   volume = 131,
    pages = {2332-2359},
      doi = {10.1086/500975},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....131.2332G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gupta2018,
   author = {{Gupta}, A. and {Yuan}, T. and {Torrey}, P. and {Vogelsberger}, M. and 
	{Martizzi}, D. and {Tran}, K.-V.~H. and {Kewley}, L.~J. and 
	{Marinacci}, F. and {Nelson}, D. and {Pillepich}, A. and {Hernquist}, L. and 
	{Genel}, S. and {Springel}, V.},
    title = "{Chemical pre-processing of cluster galaxies over the past 10 billion years in the IllustrisTNG simulations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1801.03500},
 keywords = {methods: numerical, galaxies: abundances, galaxies: clusters: general, galaxies: evolution, galaxies: groups: general},
     year = 2018,
    month = jun,
   volume = 477,
    pages = {L35-L39},
      doi = {10.1093/mnrasl/sly037},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.477L..35G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Heckman1990,
   author = {{Heckman}, T.~M. and {Armus}, L. and {Miley}, G.~K.},
    title = "{On the nature and implications of starburst-driven galactic superwinds}",
  journal = {\apjs},
 keywords = {Far Infrared Radiation, Interstellar Gas, Starburst Galaxies, Stellar Winds, Galactic Structure, Intergalactic Media, Nebulae, Optical Emission Spectroscopy, Stellar Motions},
     year = 1990,
    month = dec,
   volume = 74,
    pages = {833-868},
      doi = {10.1086/191522},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJS...74..833H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Hwang2019,
   author = {{Hwang}, H.-C. and {Barrera-Ballesteros}, J.~K. and {Heckman}, T.~M. and 
	{Rowlands}, K. and {Lin}, L. and {Rodriguez-Gomez}, V. and {Pan}, H.-A. and 
	{Hsieh}, B.-C. and {S{\'a}nchez}, S. and {Bizyaev}, D. and {S{\'a}nchez Almeida}, J. and 
	{Thilker}, D.~A. and {Lotz}, J.~M. and {Jones}, A. and {Nair}, P. and 
	{Andrews}, B.~H. and {Drory}, N.},
    title = "{Anomalously Low-metallicity Regions in MaNGA Star-forming Galaxies: Accretion Caught in Action?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1812.04614},
 keywords = {galaxies: abundances, galaxies: evolution, galaxies: statistics, surveys, techniques: imaging spectroscopy },
     year = 2019,
    month = feb,
   volume = 872,
      eid = {144},
    pages = {144},
      doi = {10.3847/1538-4357/aaf7a3},
   adsurl = {http://adsabs.harvard.edu/abs/2019ApJ...872..144H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kacprzak2016,
       author = {{Kacprzak}, Glenn G. and {van de Voort}, Freeke and {Glazebrook}, Karl and
         {Tran}, Kim-Vy H. and {Yuan}, Tiantian and {Nanayakkara}, Themiya and
         {Allen}, Rebecca J. and {Alcorn}, Leo and {Cowley}, Michael and
         {Labb{\'e}}, Ivo and {Spitler}, Lee and {Straatman}, Caroline and
         {Tomczak}, Adam},
        title = "{Cold-mode Accretion: Driving the Fundamental Mass-Metallicity Relation at z \raisebox{-0.5ex}\textasciitilde 2}",
      journal = {\apjl},
     keywords = {cosmology: observations, galaxies: abundances, galaxies: evolution, galaxies: fundamental parameters, galaxies: high-redshift, intergalactic medium, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Jul",
       volume = {826},
       number = {1},
          eid = {L11},
        pages = {L11},
          doi = {10.3847/2041-8205/826/1/L11},
archivePrefix = {arXiv},
       eprint = {1607.00014},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...826L..11K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Kauffmann2003,
   author = {{Kauffmann}, G. and {Heckman}, T.~M. and {Tremonti}, C. and 
	{Brinchmann}, J. and {Charlot}, S. and {White}, S.~D.~M. and 
	{Ridgway}, S.~E. and {Brinkmann}, J. and {Fukugita}, M. and 
	{Hall}, P.~B. and {Ivezi{\'c}}, {\v Z}. and {Richards}, G.~T. and 
	{Schneider}, D.~P.},
    title = "{The host galaxies of active galactic nuclei}",
  journal = {\mnras},
   eprint = {astro-ph/0304239},
 keywords = {galaxies: active, galaxies: Seyfert, galaxies: starburst, galaxies: stellar content, galaxies: structure},
     year = 2003,
    month = dec,
   volume = 346,
    pages = {1055-1077},
      doi = {10.1111/j.1365-2966.2003.07154.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.346.1055K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kennicutt1989,
   author = {{Kennicutt}, Jr., R.~C.},
    title = "{The star formation law in galactic disks}",
  journal = {\apj},
 keywords = {Galactic Evolution, H Alpha Line, H Ii Regions, Interstellar Gas, Star Formation Rate, Emission Spectra, Gas Dynamics, Radial Distribution, Spiral Galaxies},
     year = 1989,
    month = sep,
   volume = 344,
    pages = {685-703},
      doi = {10.1086/167834},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...344..685K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kewley2001,
   author = {{Kewley}, L.~J. and {Dopita}, M.~A. and {Sutherland}, R.~S. and 
	{Heisler}, C.~A. and {Trevena}, J.},
    title = "{Theoretical Modeling of Starburst Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/0106324},
 keywords = {Galaxies: Starburst, Radiation Mechanisms: Thermal},
     year = 2001,
    month = jul,
   volume = 556,
    pages = {121-140},
      doi = {10.1086/321545},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...556..121K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kewley2002,
   author = {{Kewley}, L.~J. and {Dopita}, M.~A.},
    title = "{Using Strong Lines to Estimate Abundances in Extragalactic H II Regions and Starburst Galaxies}",
  journal = {\apjs},
   eprint = {astro-ph/0206495},
 keywords = {Galaxies: Abundances, Galaxies: Evolution, Galaxies: Starburst, ISM: Abundances},
     year = 2002,
    month = sep,
   volume = 142,
    pages = {35-52},
      doi = {10.1086/341326},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJS..142...35K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kroupa2001,
       author = {{Kroupa}, Pavel},
        title = "{On the variation of the initial mass function}",
      journal = {\mnras},
     keywords = {BINARIES: GENERAL, STARS: FORMATION, STARS: KINEMATICS, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, GLOBULAR CLUSTERS: GENERAL, OPEN CLUSTERS AND ASSOCIATIONS: GENERAL, Astrophysics},
         year = "2001",
        month = "Apr",
       volume = {322},
       number = {2},
        pages = {231-246},
          doi = {10.1046/j.1365-8711.2001.04022.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0009005},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.322..231K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Larson1972,
   author = {{Larson}, R.~B.},
    title = "{Effect of Infalling Matter on the Heavy Element Content of a Galaxy}",
  journal = {Nature Physical Science},
     year = 1972,
    month = mar,
   volume = 236,
    pages = {7-8},
      doi = {10.1038/physci236007a0},
   adsurl = {http://adsabs.harvard.edu/abs/1972NPhS..236....7L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Larson1980,
   author = {{Larson}, R.~B. and {Tinsley}, B.~M. and {Caldwell}, C.~N.},
    title = "{The evolution of disk galaxies and the origin of S0 galaxies}",
  journal = {\apj},
 keywords = {Disk Galaxies, Galactic Evolution, Spiral Galaxies, Digital Simulation, Galactic Structure, Gas Evolution, Stellar Evolution, Stellar Magnitude},
     year = 1980,
    month = may,
   volume = 237,
    pages = {692-707},
      doi = {10.1086/157917},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...237..692L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Law2015,
   author = {{Law}, D.~R. and {Yan}, R. and {Bershady}, M.~A. and {Bundy}, K. and 
	{Cherinka}, B. and {Drory}, N. and {MacDonald}, N. and {S{\'a}nchez-Gallego}, J.~R. and 
	{Wake}, D.~A. and {Weijmans}, A.-M. and {Blanton}, M.~R. and 
	{Klaene}, M.~A. and {Moran}, S.~M. and {Sanchez}, S.~F. and 
	{Zhang}, K.},
    title = "{Observing Strategy for the SDSS-IV/MaNGA IFU Galaxy Survey}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1505.04285},
 primaryClass = "astro-ph.IM",
 keywords = {atmospheric effects, methods: observational, surveys, techniques: imaging spectroscopy},
     year = 2015,
    month = jul,
   volume = 150,
      eid = {19},
    pages = {19},
      doi = {10.1088/0004-6256/150/1/19},
   adsurl = {http://adsabs.harvard.edu/abs/2015AJ....150...19L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Law2016,
   author = {{Law}, D.~R. and {Cherinka}, B. and {Yan}, R. and {Andrews}, B.~H. and 
	{Bershady}, M.~A. and {Bizyaev}, D. and {Blanc}, G.~A. and {Blanton}, M.~R. and 
	{Bolton}, A.~S. and {Brownstein}, J.~R. and {Bundy}, K. and 
	{Chen}, Y. and {Drory}, N. and {D'Souza}, R. and {Fu}, H. and 
	{Jones}, A. and {Kauffmann}, G. and {MacDonald}, N. and {Masters}, K.~L. and 
	{Newman}, J.~A. and {Parejko}, J.~K. and {S{\'a}nchez-Gallego}, J.~R. and 
	{S{\'a}nchez}, S.~F. and {Schlegel}, D.~J. and {Thomas}, D. and 
	{Wake}, D.~A. and {Weijmans}, A.-M. and {Westfall}, K.~B. and 
	{Zhang}, K.},
    title = "{The Data Reduction Pipeline for the SDSS-IV MaNGA IFU Galaxy Survey}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1607.08619},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, surveys, techniques: imaging spectroscopy},
     year = 2016,
    month = oct,
   volume = 152,
      eid = {83},
    pages = {83},
      doi = {10.3847/0004-6256/152/4/83},
   adsurl = {http://adsabs.harvard.edu/abs/2016AJ....152...83L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lehner2013,
   author = {{Lehner}, N. and {Howk}, J.~C. and {Tripp}, T.~M. and {Tumlinson}, J. and 
	{Prochaska}, J.~X. and {O'Meara}, J.~M. and {Thom}, C. and {Werk}, J.~K. and 
	{Fox}, A.~J. and {Ribaudo}, J.},
    title = "{The Bimodal Metallicity Distribution of the Cool Circumgalactic Medium at z $\lt$\~{} 1}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1302.5424},
 keywords = {cosmology: observations, galaxies: abundances, galaxies: halos, galaxies: kinematics and dynamics},
     year = 2013,
    month = jun,
   volume = 770,
      eid = {138},
    pages = {138},
      doi = {10.1088/0004-637X/770/2/138},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...770..138L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leitherer2014,
   author = {{Leitherer}, C. and {Ekstr{\"o}m}, S. and {Meynet}, G. and {Schaerer}, D. and 
	{Agienko}, K.~B. and {Levesque}, E.~M.},
    title = "{The Effects of Stellar Rotation. II. A Comprehensive Set of Starburst99 Models}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1403.5444},
 keywords = {galaxies: starburst, galaxies: stellar content, stars: atmospheres, stars: evolution, stars: rotation},
     year = 2014,
    month = may,
   volume = 212,
      eid = {14},
    pages = {14},
      doi = {10.1088/0067-0049/212/1/14},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJS..212...14L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lilly2013,
   author = {{Lilly}, S.~J. and {Carollo}, C.~M. and {Pipino}, A. and {Renzini}, A. and 
	{Peng}, Y.},
    title = "{Gas Regulation of Galaxies: The Evolution of the Cosmic Specific Star Formation Rate, the Metallicity-Mass-Star-formation Rate Relation, and the Stellar Content of Halos}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1303.5059},
 keywords = {dark matter, galaxies: abundances, galaxies: evolution, galaxies: halos, galaxies: ISM},
     year = 2013,
    month = aug,
   volume = 772,
      eid = {119},
    pages = {119},
      doi = {10.1088/0004-637X/772/2/119},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...772..119L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@MISC{LMFIT,
       author = {{Newville}, Matthew and {Stensitzki}, Till and {Allen}, Daniel B and
         {Ingargiola}, Antonino},
        title = "{LMFIT: Non-Linear Least-Square Minimization and Curve-Fitting for Python}",
     keywords = {python, non-linear least-squares optimization, curve-fitting},
         year = "2014",
        month = "Sep",
          eid = {10.5281/zenodo.11813},
          doi = {10.5281/zenodo.11813},
    publisher = {Zenodo},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014zndo.....11813N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maiolino2019,
       author = {{Maiolino}, R. and {Mannucci}, F.},
        title = "{De re metallica: the cosmic chemical evolution of galaxies}",
      journal = {\aapr},
     keywords = {Galaxy metallicity, Chemical abundances, Galaxy evolution, Galaxy formation, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Feb",
       volume = {27},
       number = {1},
          eid = {3},
        pages = {3},
          doi = {10.1007/s00159-018-0112-2},
archivePrefix = {arXiv},
       eprint = {1811.09642},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&ARv..27....3M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mannucci2010,
   author = {{Mannucci}, F. and {Cresci}, G. and {Maiolino}, R. and {Marconi}, A. and 
	{Gnerucci}, A.},
    title = "{A fundamental relation between mass, star formation rate and metallicity in local and high-redshift galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1005.0006},
 keywords = {galaxies: abundances, galaxies: formation, galaxies: high-redshift, galaxies: starburst},
     year = 2010,
    month = nov,
   volume = 408,
    pages = {2115-2127},
      doi = {10.1111/j.1365-2966.2010.17291.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.408.2115M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mast2014,
       author = {{Mast}, D. and {Rosales-Ortega}, F.~F. and {S{\'a}nchez}, S.~F. and
         {V{\'\i}lchez}, J.~M. and {Iglesias-Paramo}, J. and {Walcher}, C.~J. and
         {Husemann}, B. and {M{\'a}rquez}, I. and {Marino}, R.~A. and
         {Kennicutt}, R.~C. and {Monreal-Ibero}, A. and {Galbany}, L. and
         {de Lorenzo-C{\'a}ceres}, A. and {Mendez-Abreu}, J. and {Kehrig}, C. and
         {del Olmo}, A. and {Rela{\~n}o}, M. and {Wisotzki}, L. and
         {M{\'a}rmol-Queralt{\'o}}, E. and {Bekerait{\`e}}, S. and
         {Papaderos}, P. and {Wild}, V. and {Aguerri}, J.~A.~L. and
         {Falc{\'o}n-Barroso}, J. and {Bomans}, D.~J. and {Ziegler}, B. and
         {Garc{\'\i}a-Lorenzo}, B. and {Bland-Hawthorn}, J. and
         {L{\'o}pez-S{\'a}nchez}, {\'A}. R. and {van de Ven}, G.},
        title = "{The effects of spatial resolution on integral field spectrograph surveys at different redshifts - The CALIFA perspective}",
      journal = {\aap},
     keywords = {techniques: spectroscopic, galaxies: abundances, stars: formation, galaxies: ISM, galaxies: stellar content, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2014",
        month = "Jan",
       volume = {561},
          eid = {A129},
        pages = {A129},
          doi = {10.1051/0004-6361/201321789},
archivePrefix = {arXiv},
       eprint = {1311.3941},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...561A.129M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Matplotlib,
  Author    = {Hunter, J. D.},
  Title     = {Matplotlib: A 2D graphics environment},
  Journal   = {Computing in Science \& Engineering},
  Volume    = {9},
  Number    = {3},
  Pages     = {90--95},
  abstract  = {Matplotlib is a 2D graphics package used for Python for
  application development, interactive scripting, and publication-quality
  image generation across user interfaces and operating systems.},
  publisher = {IEEE COMPUTER SOC},
  doi       = {10.1109/MCSE.2007.55},
  year      = 2007
}


@ARTICLE{Medling2018,
   author = {{Medling}, A.~M. and {Cortese}, L. and {Croom}, S.~M. and {Green}, A.~W. and 
	{Groves}, B. and {Hampton}, E. and {Ho}, I.-T. and {Davies}, L.~J.~M. and 
	{Kewley}, L.~J. and {Moffett}, A.~J. and {Schaefer}, A.~L. and 
	{Taylor}, E. and {Zafar}, T. and {Bekki}, K. and {Bland-Hawthorn}, J. and 
	{Bloom}, J.~V. and {Brough}, S. and {Bryant}, J.~J. and {Catinella}, B. and 
	{Cecil}, G. and {Colless}, M. and {Couch}, W.~J. and {Drinkwater}, M.~J. and 
	{Driver}, S.~P. and {Federrath}, C. and {Foster}, C. and {Goldstein}, G. and 
	{Goodwin}, M. and {Hopkins}, A. and {Lawrence}, J.~S. and {Leslie}, S.~K. and 
	{Lewis}, G.~F. and {Lorente}, N.~P.~F. and {Owers}, M.~S. and 
	{McDermid}, R. and {Richards}, S.~N. and {Sharp}, R. and {Scott}, N. and 
	{Sweet}, S.~M. and {Taranu}, D.~S. and {Tescari}, E. and {Tonini}, C. and 
	{van de Sande}, J. and {Walcher}, C.~J. and {Wright}, A.},
    title = "{The SAMI Galaxy Survey: spatially resolving the main sequence of star formation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1801.04283},
 keywords = {surveys, galaxies: evolution, galaxies: star formation},
     year = 2018,
    month = apr,
   volume = 475,
    pages = {5194-5214},
      doi = {10.1093/mnras/sty127},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.475.5194M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Moran2012,
   author = {{Moran}, S.~M. and {Heckman}, T.~M. and {Kauffmann}, G. and 
	{Dav{\'e}}, R. and {Catinella}, B. and {Brinchmann}, J. and 
	{Wang}, J. and {Schiminovich}, D. and {Saintonge}, A. and {Gracia-Carpio}, J. and 
	{Tacconi}, L. and {Giovanelli}, R. and {Haynes}, M. and {Fabello}, S. and 
	{Hummels}, C. and {Lemonias}, J. and {Wu}, R.},
    title = "{The GALEX Arecibo SDSS Survey. V. The Relation between the H I Content of Galaxies and Metal Enrichment at Their Outskirts}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1112.1084},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: ISM, galaxies: star formation, galaxies: stellar content},
     year = 2012,
    month = jan,
   volume = 745,
      eid = {66},
    pages = {66},
      doi = {10.1088/0004-637X/745/1/66},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...745...66M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Navarro1997,
   author = {{Navarro}, J.~F. and {Frenk}, C.~S. and {White}, S.~D.~M.},
    title = "{A Universal Density Profile from Hierarchical Clustering}",
  journal = {\apj},
   eprint = {astro-ph/9611107},
 keywords = {Cosmology: Theory, Cosmology: Dark Matter, Galaxies: Halos, Methods: Numerical},
     year = 1997,
    month = dec,
   volume = 490,
    pages = {493-508},
      doi = {10.1086/304888},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...490..493N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oppenheimer2010,
   author = {{Oppenheimer}, B.~D. and {Dav{\'e}}, R. and {Kere{\v s}}, D. and 
	{Fardal}, M. and {Katz}, N. and {Kollmeier}, J.~A. and {Weinberg}, D.~H.
	},
    title = "{Feedback and recycled wind accretion: assembling the z = 0 galaxy mass function}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0912.0519},
 keywords = {hydrodynamics, methods: numerical, galaxies: evolution, galaxies: formation, intergalactic medium, galaxies: luminosity function, mass function},
     year = 2010,
    month = aug,
   volume = 406,
    pages = {2325-2338},
      doi = {10.1111/j.1365-2966.2010.16872.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.406.2325O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parikh2018,
   author = {{Parikh}, T. and {Thomas}, D. and {Maraston}, C. and {Westfall}, K.~B. and 
	{Goddard}, D. and {Lian}, J. and {Meneses-Goytia}, S. and {Jones}, A. and 
	{Vaughan}, S. and {Andrews}, B.~H. and {Bershady}, M. and {Bizyaev}, D. and 
	{Brinkmann}, J. and {Brownstein}, J.~R. and {Bundy}, K. and 
	{Drory}, N. and {Emsellem}, E. and {Law}, D.~R. and {Newman}, J.~A. and 
	{Roman-Lopes}, A. and {Wake}, D. and {Yan}, R. and {Zheng}, Z.
	},
    title = "{SDSS-IV MaNGA: the spatially resolved stellar initial mass function in {\tilde}400 early-type galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1803.08515},
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: stellar content},
     year = 2018,
    month = jul,
   volume = 477,
    pages = {3954-3982},
      doi = {10.1093/mnras/sty785},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.477.3954P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Pasquali2012,
   author = {{Pasquali}, A. and {Gallazzi}, A. and {van den Bosch}, F.~C.
	},
    title = "{The gas-phase metallicity of central and satellite galaxies in the Sloan Digital Sky Survey}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1206.3458},
 keywords = {galaxies: abundances, galaxies: evolution, galaxies: fundamental parameters, galaxies: groups: general, galaxies: star formation },
     year = 2012,
    month = sep,
   volume = 425,
    pages = {273-286},
      doi = {10.1111/j.1365-2966.2012.21454.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425..273P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Peeples2011,
   author = {{Peeples}, M.~S. and {Shankar}, F.},
    title = "{Constraints on star formation driven galaxy winds from the mass-metallicity relation at z= 0}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1007.3743},
 primaryClass = "astro-ph.CO",
 keywords = {ISM: abundances, ISM: jets and outflows, galaxies: abundances, galaxies: evolution, galaxies: fundamental parameters, galaxies: ISM},
     year = 2011,
    month = nov,
   volume = 417,
    pages = {2962-2981},
      doi = {10.1111/j.1365-2966.2011.19456.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.417.2962P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pellegrini2019,
       author = {{Pellegrini}, E.~W. and {Reissl}, S. and {Rahner}, D. and
         {Klessen}, R.~S. and {Glover}, S.~C.~O. and {Pakmor}, R. and
         {Herrera-Camus}, R. and {Grand}, R.~J.~J.},
        title = "{WARPFIELD Population Synthesis: The physics of (extra-)Galactic star formation and feedback driven cloud structure and emission from sub-to-kpc scales}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2019",
        month = "May",
          eid = {arXiv:1905.04158},
        pages = {arXiv:1905.04158},
archivePrefix = {arXiv},
       eprint = {1905.04158},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190504158P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Peng2012,
   author = {{Peng}, Y.-j. and {Lilly}, S.~J. and {Renzini}, A. and {Carollo}, M.
	},
    title = "{Mass and Environment as Drivers of Galaxy Evolution. II. The Quenching of Satellite Galaxies as the Origin of Environmental Effects}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.2546},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: groups: general, galaxies: luminosity function, mass function},
     year = 2012,
    month = sep,
   volume = 757,
      eid = {4},
    pages = {4},
      doi = {10.1088/0004-637X/757/1/4},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...757....4P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Peng2014,
   author = {{Peng}, Y.-j. and {Maiolino}, R.},
    title = "{The dependence of the galaxy mass-metallicity relation on environment and the implied metallicity of the IGM}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1311.1816},
 keywords = {galaxies: abundances, galaxies: evolution, galaxies: formation, galaxies: fundamental parameters},
     year = 2014,
    month = feb,
   volume = 438,
    pages = {262-270},
      doi = {10.1093/mnras/stt2175},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438..262P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Peng2015,
   author = {{Peng}, Y. and {Maiolino}, R. and {Cochrane}, R.},
    title = "{Strangulation as the primary mechanism for shutting down star formation in galaxies}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1505.03143},
     year = 2015,
    month = may,
   volume = 521,
    pages = {192-195},
      doi = {10.1038/nature14439},
   adsurl = {http://adsabs.harvard.edu/abs/2015Natur.521..192P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pettini2004,
   author = {{Pettini}, M. and {Pagel}, B.~E.~J.},
    title = "{[OIII]/[NII] as an abundance indicator at high redshift}",
  journal = {\mnras},
   eprint = {astro-ph/0401128},
 keywords = {ISM: abundances, HII regions, galaxies: abundances},
     year = 2004,
    month = mar,
   volume = 348,
    pages = {L59-L63},
      doi = {10.1111/j.1365-2966.2004.07591.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.348L..59P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Poetrodjojo2018,
   author = {{Poetrodjojo}, H. and {Groves}, B. and {Kewley}, L.~J. and {Medling}, A.~M. and 
	{Sweet}, S.~M. and {van de Sande}, J. and {Sanchez}, S.~F. and 
	{Bland-Hawthorn}, J. and {Brough}, S. and {Bryant}, J.~J. and 
	{Cortese}, L. and {Croom}, S.~M. and {L{\'o}pez-S{\'a}nchez}, {\'A}.~R. and 
	{Richards}, S.~N. and {Zafar}, T. and {Lawrence}, J.~S. and 
	{Lorente}, N.~P.~F. and {Owers}, M.~S. and {Scott}, N.},
    title = "{The SAMI Galaxy Survey: Spatially resolved metallicity and ionization mapping}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1807.01522},
 keywords = {galaxies: abundances, galaxies: ISM},
     year = 2018,
    month = oct,
   volume = 479,
    pages = {5235-5265},
      doi = {10.1093/mnras/sty1782},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.479.5235P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Prochaska2017,
   author = {{Prochaska}, J.~X. and {Werk}, J.~K. and {Worseck}, G. and {Tripp}, T.~M. and 
	{Tumlinson}, J. and {Burchett}, J.~N. and {Fox}, A.~J. and {Fumagalli}, M. and 
	{Lehner}, N. and {Peeples}, M.~S. and {Tejos}, N.},
    title = "{The COS-Halos Survey: Metallicities in the Low-redshift Circumgalactic Medium}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1702.02618},
 keywords = {galaxies: halos},
     year = 2017,
    month = mar,
   volume = 837,
      eid = {169},
    pages = {169},
      doi = {10.3847/1538-4357/aa6007},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...837..169P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Quirk1973,
       author = {{Quirk}, William J. and {Tinsley}, Beatrice M.},
        title = "{Star Formation and Evolution in Spiral Galaxies}",
      journal = {\apj},
         year = "1973",
        month = "Jan",
       volume = {179},
        pages = {69-84},
          doi = {10.1086/151847},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1973ApJ...179...69Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Renzini2014,
   author = {{Renzini}, A. and {Andreon}, S.},
    title = "{Chemical evolution on the scale of clusters of galaxies: a conundrum?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1409.0307},
 keywords = {galaxies: abundances, galaxies: clusters: general, galaxies: clusters: intracluster medium},
     year = 2014,
    month = nov,
   volume = 444,
    pages = {3581-3591},
      doi = {10.1093/mnras/stu1689},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.444.3581R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Robotham2011,
       author = {{Robotham}, A.~S.~G. and {Norberg}, P. and {Driver}, S.~P. and
         {Baldry}, I.~K. and {Bamford}, S.~P. and {Hopkins}, A.~M. and
         {Liske}, J. and {Loveday}, J. and {Merson}, A. and {Peacock}, J.~A. and
         {Brough}, S. and {Cameron}, E. and {Conselice}, C.~J. and
         {Croom}, S.~M. and {Frenk}, C.~S. and {Gunawardhana}, M. and
         {Hill}, D.~T. and {Jones}, D.~H. and {Kelvin}, L.~S. and {Kuijken}, K. and
         {Nichol}, R.~C. and {Parkinson}, H.~R. and {Pimbblet}, K.~A. and
         {Phillipps}, S. and {Popescu}, C.~C. and {Prescott}, M. and
         {Sharp}, R.~G. and {Sutherland}, W.~J. and {Taylor}, E.~N. and
         {Thomas}, D. and {Tuffs}, R.~J. and {van Kampen}, E. and
         {Wijesinghe}, D.},
        title = "{Galaxy and Mass Assembly (GAMA): the GAMA galaxy group catalogue (G$^{3}$Cv1)}",
      journal = {\mnras},
     keywords = {galaxies: groups: general, galaxies: haloes, dark matter, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2011",
        month = "Oct",
       volume = {416},
       number = {4},
        pages = {2640-2668},
          doi = {10.1111/j.1365-2966.2011.19217.x},
archivePrefix = {arXiv},
       eprint = {1106.1994},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.416.2640R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{RosalesOrtega2012,
   author = {{Rosales-Ortega}, F.~F. and {S{\'a}nchez}, S.~F. and {Iglesias-P{\'a}ramo}, J. and 
	{D{\'{\i}}az}, A.~I. and {V{\'{\i}}lchez}, J.~M. and {Bland-Hawthorn}, J. and 
	{Husemann}, B. and {Mast}, D.},
    title = "{A New Scaling Relation for H II Regions in Spiral Galaxies: Unveiling the True Nature of the Mass-Metallicity Relation}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1207.6216},
 keywords = {galaxies: abundances, galaxies: fundamental parameters, galaxies: ISM, galaxies: stellar content, techniques: imaging spectroscopy},
     year = 2012,
    month = sep,
   volume = 756,
      eid = {L31},
    pages = {L31},
      doi = {10.1088/2041-8205/756/2/L31},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...756L..31R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rubin2012,
       author = {{Rubin}, Kate H.~R. and {Prochaska}, J. Xavier and {Koo}, David C. and
         {Phillips}, Andrew C.},
        title = "{The Direct Detection of Cool, Metal-enriched Gas Accretion onto Galaxies at z \raisebox{-0.5ex}\textasciitilde 0.5}",
      journal = {\apjl},
     keywords = {galaxies: evolution, galaxies: halos, galaxies: ISM, quasars: absorption lines, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2012",
        month = "Mar",
       volume = {747},
       number = {2},
          eid = {L26},
        pages = {L26},
          doi = {10.1088/2041-8205/747/2/L26},
archivePrefix = {arXiv},
       eprint = {1110.0837},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...747L..26R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SanchezBlazquez2006,
   author = {{S{\'a}nchez-Bl{\'a}zquez}, P. and {Peletier}, R.~F. and {Jim{\'e}nez-Vicente}, J. and 
	{Cardiel}, N. and {Cenarro}, A.~J. and {Falc{\'o}n-Barroso}, J. and 
	{Gorgas}, J. and {Selam}, S. and {Vazdekis}, A.},
    title = "{Medium-resolution Isaac Newton Telescope library of empirical spectra}",
  journal = {\mnras},
   eprint = {astro-ph/0607009},
 keywords = {atlases: stars: fundamental parameters: galaxies: stellar content, atlases, stars: fundamental parameters, galaxies: stellar content},
     year = 2006,
    month = sep,
   volume = 371,
    pages = {703-718},
      doi = {10.1111/j.1365-2966.2006.10699.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.371..703S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sanchez2012,
   author = {{S{\'a}nchez}, S.~F. and {Kennicutt}, R.~C. and {Gil de Paz}, A. and 
	{van de Ven}, G. and {V{\'{\i}}lchez}, J.~M. and {Wisotzki}, L. and 
	{Walcher}, C.~J. and {Mast}, D. and {Aguerri}, J.~A.~L. and 
	{Albiol-P{\'e}rez}, S. and {Alonso-Herrero}, A. and {Alves}, J. and 
	{Bakos}, J. and {Bart{\'a}kov{\'a}}, T. and {Bland-Hawthorn}, J. and 
	{Boselli}, A. and {Bomans}, D.~J. and {Castillo-Morales}, A. and 
	{Cortijo-Ferrero}, C. and {de Lorenzo-C{\'a}ceres}, A. and {Del Olmo}, A. and 
	{Dettmar}, R.-J. and {D{\'{\i}}az}, A. and {Ellis}, S. and {Falc{\'o}n-Barroso}, J. and 
	{Flores}, H. and {Gallazzi}, A. and {Garc{\'{\i}}a-Lorenzo}, B. and 
	{Gonz{\'a}lez Delgado}, R. and {Gruel}, N. and {Haines}, T. and 
	{Hao}, C. and {Husemann}, B. and {Igl{\'e}sias-P{\'a}ramo}, J. and 
	{Jahnke}, K. and {Johnson}, B. and {Jungwiert}, B. and {Kalinova}, V. and 
	{Kehrig}, C. and {Kupko}, D. and {L{\'o}pez-S{\'a}nchez}, {\'A}.~R. and 
	{Lyubenova}, M. and {Marino}, R.~A. and {M{\'a}rmol-Queralt{\'o}}, E. and 
	{M{\'a}rquez}, I. and {Masegosa}, J. and {Meidt}, S. and {Mendez-Abreu}, J. and 
	{Monreal-Ibero}, A. and {Montijo}, C. and {Mour{\~a}o}, A.~M. and 
	{Palacios-Navarro}, G. and {Papaderos}, P. and {Pasquali}, A. and 
	{Peletier}, R. and {P{\'e}rez}, E. and {P{\'e}rez}, I. and {Quirrenbach}, A. and 
	{Rela{\~n}o}, M. and {Rosales-Ortega}, F.~F. and {Roth}, M.~M. and 
	{Ruiz-Lara}, T. and {S{\'a}nchez-Bl{\'a}zquez}, P. and {Sengupta}, C. and 
	{Singh}, R. and {Stanishev}, V. and {Trager}, S.~C. and {Vazdekis}, A. and 
	{Viironen}, K. and {Wild}, V. and {Zibetti}, S. and {Ziegler}, B.
	},
    title = "{CALIFA, the Calar Alto Legacy Integral Field Area survey. I. Survey presentation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1111.0962},
 keywords = {techniques: spectroscopic, galaxies: active, galaxies: evolution, surveys, galaxies: ISM, galaxies: stellar content},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A8},
    pages = {A8},
      doi = {10.1051/0004-6361/201117353},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538A...8S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sanchez2016a,
   author = {{S{\'a}nchez}, S.~F. and {P{\'e}rez}, E. and {S{\'a}nchez-Bl{\'a}zquez}, P. and 
	{Gonz{\'a}lez}, J.~J. and {Ros{\'a}lez-Ortega}, F.~F. and {Cano-D{\'{\i}} az}, M. and 
	{L{\'o}pez-Cob{\'a}}, C. and {Marino}, R.~A. and {Gil de Paz}, A. and 
	{Moll{\'a}}, M. and {L{\'o}pez-S{\'a}nchez}, A.~R. and {Ascasibar}, Y. and 
	{Barrera-Ballesteros}, J.},
    title = "{Pipe3D, a pipeline to analyze Integral Field Spectroscopy Data: I. New fitting philosophy of FIT3D}",
  journal = {\rmxaa},
archivePrefix = "arXiv",
   eprint = {1509.08552},
 primaryClass = "astro-ph.IM",
 keywords = {galaxies: ISM, techniques: spectroscopic},
     year = 2016,
    month = apr,
   volume = 52,
    pages = {21-53},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2016RMxAA..52...21S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Sanchez2016b,
   author = {{S{\'a}nchez}, S.~F. and {P{\'e}rez}, E. and {S{\'a}nchez-Bl{\'a}zquez}, P. and 
	{Garc{\'{\i}}a-Benito}, R. and {Ibarra-Mede}, H.~J. and {Gonz{\'a}lez}, J.~J. and 
	{Rosales-Ortega}, F.~F. and {S{\'a}nchez-Menguiano}, L. and 
	{Ascasibar}, Y. and {Bitsakis}, T. and {Law}, D. and {Cano-D{\'{\i}}az}, M. and 
	{L{\'o}pez-Cob{\'a}}, C. and {Marino}, R.~A. and {Gil de Paz}, A. and 
	{L{\'o}pez-S{\'a}nchez}, A.~R. and {Barrera-Ballesteros}, J. and 
	{Galbany}, L. and {Mast}, D. and {Abril-Melgarejo}, V. and {Roman-Lopes}, A.
	},
    title = "{Pipe3D, a pipeline to analyze Integral Field Spectroscopy Data: II. Analysis sequence and CALIFA dataproducts}",
  journal = {\rmxaa},
archivePrefix = "arXiv",
   eprint = {1602.01830},
 primaryClass = "astro-ph.IM",
 keywords = {galaxies: structure, methods: data analysis, surveys, techniques: spectroscopic},
     year = 2016,
    month = apr,
   volume = 52,
    pages = {171-220},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2016RMxAA..52..171S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sanchez2018,
       author = {{S{\'a}nchez}, S.~F. and {Avila-Reese}, V. and {Hernandez-Toledo}, H. and
         {Cortes-Su{\'a}rez}, E. and {Rodr{\'\i}guez-Puebla}, A. and
         {Ibarra-Medel}, H. and {Cano-D{\'\i}az}, M. and
         {Barrera-Ballesteros}, J.~K. and {Negrete}, C.~A. and {Calette}, A.~R. and
         {de Lorenzo-C{\'a}ceres}, A. and {Ortega-Minakata}, R.~A. and
         {Aquino}, E. and {Valenzuela}, O. and {Clemente}, J.~C. and
         {Storchi-Bergmann}, T. and {Riffel}, R. and {Schimoia}, J. and
         {Riffel}, R.~A. and {Rembold}, S.~B. and {Brownstein}, J.~R. and
         {Pan}, K. and {Yates}, R. and {Mallmann}, N. and {Bitsakis}, T.},
        title = "{SDSS IV MaNGA - Properties of AGN Host Galaxies}",
      journal = {\rmxaa},
     keywords = {catalogues, galaxies: active, galaxies: evolution, galaxies: nuclei, galaxies: star formation, techniques: imaging spectroscopy, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Apr",
       volume = {54},
        pages = {217-260},
archivePrefix = {arXiv},
       eprint = {1709.05438},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018RMxAA..54..217S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Sanchez2019,
   author = {{S{\'a}nchez}, S.~F. and {Barrera-Ballesteros}, J.~K. and {L{\'o}pez-Cob{\'a}}, C. and 
	{Brough}, S. and {Bryant}, J.~J. and {Bland-Hawthorn}, J. and 
	{Croom}, S.~M. and {van de Sande}, J. and {Cortese}, L. and 
	{Goodwin}, M. and {Lawrence}, J.~S. and {L{\'o}pez-S{\'a}nchez}, A.~R. and 
	{Sweet}, S.~M. and {Owers}, M.~S. and {Richards}, S.~N. and 
	{Walcher}, C.~J.},
    title = "{The SAMI Galaxy Survey: Exploring the gas-phase Mass-Metallicity Relation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1812.11263},
 keywords = {galaxies: abundances, galaxies: evolution, galaxies: ISM, techniques: spectroscopic},
     year = 2019,
    month = jan,
      doi = {10.1093/mnras/stz019},
   adsurl = {http://adsabs.harvard.edu/abs/2019MNRAS.tmp...29S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schaefer2019,
       author = {{Schaefer}, A.~L. and {Croom}, S.~M. and {Scott}, N. and {Brough}, S. and
         {Allen}, J.~T. and {Bekki}, K. and {Bland-Hawthorn}, J. and
         {Bloom}, J.~V. and {Bryant}, J.~J. and {Cortese}, L.},
        title = "{The SAMI Galaxy Survey: observing the environmental quenching of star formation in GAMA groups}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: interactions, galaxies: star formation, galaxies: structure, galaxies: groups: general, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Mar",
       volume = {483},
       number = {3},
        pages = {2851-2870},
          doi = {10.1093/mnras/sty3258},
archivePrefix = {arXiv},
       eprint = {1811.11676},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483.2851S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Smee2013,
   author = {{Smee}, S.~A. and {Gunn}, J.~E. and {Uomoto}, A. and {Roe}, N. and 
	{Schlegel}, D. and {Rockosi}, C.~M. and {Carr}, M.~A. and {Leger}, F. and 
	{Dawson}, K.~S. and {Olmstead}, M.~D. and {Brinkmann}, J. and 
	{Owen}, R. and {Barkhouser}, R.~H. and {Honscheid}, K. and {Harding}, P. and 
	{Long}, D. and {Lupton}, R.~H. and {Loomis}, C. and {Anderson}, L. and 
	{Annis}, J. and {Bernardi}, M. and {Bhardwaj}, V. and {Bizyaev}, D. and 
	{Bolton}, A.~S. and {Brewington}, H. and {Briggs}, J.~W. and 
	{Burles}, S. and {Burns}, J.~G. and {Castander}, F.~J. and {Connolly}, A. and 
	{Davenport}, J.~R.~A. and {Ebelke}, G. and {Epps}, H. and {Feldman}, P.~D. and 
	{Friedman}, S.~D. and {Frieman}, J. and {Heckman}, T. and {Hull}, C.~L. and 
	{Knapp}, G.~R. and {Lawrence}, D.~M. and {Loveday}, J. and {Mannery}, E.~J. and 
	{Malanushenko}, E. and {Malanushenko}, V. and {Merrelli}, A.~J. and 
	{Muna}, D. and {Newman}, P.~R. and {Nichol}, R.~C. and {Oravetz}, D. and 
	{Pan}, K. and {Pope}, A.~C. and {Ricketts}, P.~G. and {Shelden}, A. and 
	{Sandford}, D. and {Siegmund}, W. and {Simmons}, A. and {Smith}, D.~S. and 
	{Snedden}, S. and {Schneider}, D.~P. and {SubbaRao}, M. and 
	{Tremonti}, C. and {Waddell}, P. and {York}, D.~G.},
    title = "{The Multi-object, Fiber-fed Spectrographs for the Sloan Digital Sky Survey and the Baryon Oscillation Spectroscopic Survey}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1208.2233},
 primaryClass = "astro-ph.IM",
 keywords = {cosmology: observations, instrumentation: spectrographs, surveys },
     year = 2013,
    month = aug,
   volume = 146,
      eid = {32},
    pages = {32},
      doi = {10.1088/0004-6256/146/2/32},
   adsurl = {http://adsabs.harvard.edu/abs/2013AJ....146...32S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Smirnov1939,
  title={On the estimation of the discrepancy between empirical curves of distribution for two independent samples},
  author={Smirnov, Nikolai V},
  journal={Bull. Math. Univ. Moscou},
  volume={2},
  number={2},
  pages={3--14},
  year={1939}
}


@ARTICLE{Tempel2017,
   author = {{Tempel}, E. and {Tuvikene}, T. and {Kipper}, R. and {Libeskind}, N.~I.
	},
    title = "{Merging groups and clusters of galaxies from the SDSS data. The catalogue of groups and potentially merging systems}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1704.04477},
 keywords = {catalogs, galaxies: groups: general, galaxies: clusters: general, large-scale structure of Universe},
     year = 2017,
    month = jun,
   volume = 602,
      eid = {A100},
    pages = {A100},
      doi = {10.1051/0004-6361/201730499},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...602A.100T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tremonti2004,
   author = {{Tremonti}, C.~A. and {Heckman}, T.~M. and {Kauffmann}, G. and 
	{Brinchmann}, J. and {Charlot}, S. and {White}, S.~D.~M. and 
	{Seibert}, M. and {Peng}, E.~W. and {Schlegel}, D.~J. and {Uomoto}, A. and 
	{Fukugita}, M. and {Brinkmann}, J.},
    title = "{The Origin of the Mass-Metallicity Relation: Insights from 53,000 Star-forming Galaxies in the Sloan Digital Sky Survey}",
  journal = {\apj},
   eprint = {astro-ph/0405537},
 keywords = {Galaxies: Abundances, Galaxies: Evolution, Galaxies: Fundamental Parameters, Galaxies: Statistics},
     year = 2004,
    month = oct,
   volume = 613,
    pages = {898-913},
      doi = {10.1086/423264},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...613..898T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Trussler2018,
       author = {{Trussler}, James and {Maiolino}, Roberto and {Maraston}, Claudia and
         {Peng}, Yingjie and {Thomas}, Daniel and {Goddard}, Daniel and
         {Lian}, Jianhui},
        title = "{Starvation as the primary quenching mechanism in galaxies}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Nov",
          eid = {arXiv:1811.09283},
        pages = {arXiv:1811.09283},
archivePrefix = {arXiv},
       eprint = {1811.09283},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv181109283T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vincenzo2016,
       author = {{Vincenzo}, F. and {Matteucci}, F. and {Belfiore}, F. and {Maiolino}, R.},
        title = "{Modern yields per stellar generation: the effect of the IMF}",
      journal = {\mnras},
     keywords = {stars: abundances, ISM: abundances, galaxies: evolution, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Feb",
       volume = {455},
       number = {4},
        pages = {4183-4190},
          doi = {10.1093/mnras/stv2598},
archivePrefix = {arXiv},
       eprint = {1503.08300},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.455.4183V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vonderlinden2010,
   author = {{von der Linden}, A. and {Wild}, V. and {Kauffmann}, G. and 
	{White}, S.~D.~M. and {Weinmann}, S.},
    title = "{Star formation and AGN activity in SDSS cluster galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0909.3522},
 keywords = {galaxies: clusters: general, galaxies: evolution, galaxies: statistics, galaxies: stellar content},
     year = 2010,
    month = may,
   volume = 404,
    pages = {1231-1246},
      doi = {10.1111/j.1365-2966.2010.16375.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.404.1231V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wake2017,
       author = {{Wake}, David A. and {Bundy}, Kevin and {Diamond-Stanic}, Aleksandar M. and
         {Yan}, Renbin and {Blanton}, Michael R. and {Bershady}, Matthew A. and
         {S{\'a}nchez-Gallego}, Jos{\'e} R. and {Drory}, Niv and {Jones}, Amy and
         {Kauffmann}, Guinevere},
        title = "{The SDSS-IV MaNGA Sample: Design, Optimization, and Usage Considerations}",
      journal = {\aj},
     keywords = {galaxies: evolution, galaxies: general, galaxies: statistics, surveys, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Sep",
       volume = {154},
       number = {3},
          eid = {86},
        pages = {86},
          doi = {10.3847/1538-3881/aa7ecc},
archivePrefix = {arXiv},
       eprint = {1707.02989},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154...86W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Westfall2019,
   author = {{Westfall}, K.~B. and {Cappellari}, M. and {Bershady}, M.~A. and 
	{Bundy}, K. and {Belfiore}, F. and {Ji}, X. and {Law}, D.~R. and 
	{Schaefer}, A. and {Shetty}, S. and {Tremonti}, C.~A. and {Yan}, R. and 
	{Andrews}, B.~H. and {Brownstein}, J.~R. and {Cherinka}, B. and 
	{Coccato}, L. and {Drory}, N. and {Maraston}, C. and {Parikh}, T. and 
	{S{\'a}nchez-Gallego}, J.~R. and {Thomas}, D. and {Weijmans}, A.-M. and 
	{Barrera-Ballesteros}, J. and {Du}, C. and {Goddard}, D. and 
	{Li}, N. and {Masters}, K. and {Ibarra Medel}, H.~J. and {S{\'a}nchez}, S.~F. and 
	{Yang}, M. and {Zheng}, Z. and {Zhou}, S.},
    title = "{The Data Analysis Pipeline for the SDSS-IV MaNGA IFU Galaxy Survey: Overview}",
  journal = {arXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1901.00856},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2019,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2019arXiv190100856W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Wu2017,
       author = {{Wu}, Po-Feng and {Zahid}, H. Jabran and {Hwang}, Ho Seong and
         {Geller}, Margaret J.},
        title = "{The dependence of the mass-metallicity relation on large-scale environment}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: evolution, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Jun",
       volume = {468},
       number = {2},
        pages = {1881-1892},
          doi = {10.1093/mnras/stx597},
archivePrefix = {arXiv},
       eprint = {1702.03323},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.468.1881W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Wuyts2011,
   author = {{Wuyts}, S. and {F{\"o}rster Schreiber}, N.~M. and {van der Wel}, A. and 
	{Magnelli}, B. and {Guo}, Y. and {Genzel}, R. and {Lutz}, D. and 
	{Aussel}, H. and {Barro}, G. and {Berta}, S. and {Cava}, A. and 
	{Graci{\'a}-Carpio}, J. and {Hathi}, N.~P. and {Huang}, K.-H. and 
	{Kocevski}, D.~D. and {Koekemoer}, A.~M. and {Lee}, K.-S. and 
	{Le Floc'h}, E. and {McGrath}, E.~J. and {Nordon}, R. and {Popesso}, P. and 
	{Pozzi}, F. and {Riguccini}, L. and {Rodighiero}, G. and {Saintonge}, A. and 
	{Tacconi}, L.},
    title = "{Galaxy Structure and Mode of Star Formation in the SFR-Mass Plane from z \~{} 2.5 to z \~{} 0.1}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1107.0317},
 keywords = {galaxies: high-redshift, galaxies: stellar content, galaxies: structure},
     year = 2011,
    month = dec,
   volume = 742,
      eid = {96},
    pages = {96},
      doi = {10.1088/0004-637X/742/2/96},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...742...96W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yan2016,
   author = {{Yan}, R. and {Bundy}, K. and {Law}, D.~R. and {Bershady}, M.~A. and 
	{Andrews}, B. and {Cherinka}, B. and {Diamond-Stanic}, A.~M. and 
	{Drory}, N. and {MacDonald}, N. and {S{\'a}nchez-Gallego}, J.~R. and 
	{Thomas}, D. and {Wake}, D.~A. and {Weijmans}, A.-M. and {Westfall}, K.~B. and 
	{Zhang}, K. and {Arag{\'o}n-Salamanca}, A. and {Belfiore}, F. and 
	{Bizyaev}, D. and {Blanc}, G.~A. and {Blanton}, M.~R. and {Brownstein}, J. and 
	{Cappellari}, M. and {D'Souza}, R. and {Emsellem}, E. and {Fu}, H. and 
	{Gaulme}, P. and {Graham}, M.~T. and {Goddard}, D. and {Gunn}, J.~E. and 
	{Harding}, P. and {Jones}, A. and {Kinemuchi}, K. and {Li}, C. and 
	{Li}, H. and {Maiolino}, R. and {Mao}, S. and {Maraston}, C. and 
	{Masters}, K. and {Merrifield}, M.~R. and {Oravetz}, D. and 
	{Pan}, K. and {Parejko}, J.~K. and {Sanchez}, S.~F. and {Schlegel}, D. and 
	{Simmons}, A. and {Thanjavur}, K. and {Tinker}, J. and {Tremonti}, C. and 
	{van den Bosch}, R. and {Zheng}, Z.},
    title = "{SDSS-IV MaNGA IFS Galaxy Survey{\mdash}Survey Design, Execution, and Initial Data Quality}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1607.08613},
 keywords = {galaxies: evolution, galaxies: general, surveys, techniques: imaging spectroscopy},
     year = 2016,
    month = dec,
   volume = 152,
      eid = {197},
    pages = {197},
      doi = {10.3847/0004-6256/152/6/197},
   adsurl = {http://adsabs.harvard.edu/abs/2016AJ....152..197Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yuan2013,
       author = {{Yuan}, T. -T. and {Kewley}, L.~J. and {Richard}, J.},
        title = "{The Metallicity Evolution of Star-forming Galaxies from Redshift 0 to 3: Combining Magnitude-limited Survey with Gravitational Lensing}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: evolution, galaxies: high-redshift, gravitational lensing: strong, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2013",
        month = "Jan",
       volume = {763},
       number = {1},
          eid = {9},
        pages = {9},
          doi = {10.1088/0004-637X/763/1/9},
archivePrefix = {arXiv},
       eprint = {1211.6423},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...763....9Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Zahid2012,
       author = {{Zahid}, H.~J. and {Dima}, G.~I. and {Kewley}, L.~J. and {Erb}, D.~K. and
         {Dav{\'e}}, R.},
        title = "{A Census of Oxygen in Star-forming Galaxies: An Empirical Model Linking Metallicities, Star Formation Rates, and Outflows}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: evolution, galaxies: formation, galaxies: high-redshift, galaxies: ISM, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Sep",
       volume = {757},
       number = {1},
          eid = {54},
        pages = {54},
          doi = {10.1088/0004-637X/757/1/54},
archivePrefix = {arXiv},
       eprint = {1207.5509},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...757...54Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Zhang2017,
   author = {{Zhang}, K. and {Yan}, R. and {Bundy}, K. and {Bershady}, M. and 
	{Haffner}, L.~M. and {Walterbos}, R. and {Maiolino}, R. and 
	{Tremonti}, C. and {Thomas}, D. and {Drory}, N. and {Jones}, A. and 
	{Belfiore}, F. and {S{\'a}nchez}, S.~F. and {Diamond-Stanic}, A.~M. and 
	{Bizyaev}, D. and {Nitschelm}, C. and {Andrews}, B. and {Brinkmann}, J. and 
	{Brownstein}, J.~R. and {Cheung}, E. and {Li}, C. and {Law}, D.~R. and 
	{Roman Lopes}, A. and {Oravetz}, D. and {Pan}, K. and {Storchi Bergmann}, T. and 
	{Simmons}, A.},
    title = "{SDSS-IV MaNGA: the impact of diffuse ionized gas on emission-line ratios, interpretation of diagnostic diagrams and gas metallicity measurements}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1612.02000},
 keywords = {galaxies: abundances, galaxies: active, galaxies: evolution, galaxies: fundamental parameters, galaxies: ISM},
     year = 2017,
    month = apr,
   volume = 466,
    pages = {3217-3243},
      doi = {10.1093/mnras/stw3308},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.466.3217Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Zhu2017,
   author = {{Zhu}, G.~B. and {Barrera-Ballesteros}, J.~K. and {Heckman}, T.~M. and 
	{Zakamska}, N.~L. and {S{\'a}nchez}, S.~F. and {Yan}, R. and 
	{Brinkmann}, J.},
    title = "{A local leaky-box model for the local stellar surface density-gas surface density-gas phase metallicity relation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1701.00003},
 keywords = {galaxies: abundances, galaxies: evolution, galaxies: spiral, galaxies: star formation},
     year = 2017,
    month = jul,
   volume = 468,
    pages = {4494-4501},
      doi = {10.1093/mnras/stx740},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.468.4494Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





